Inroads into Autonomous Network Defence using Explained Reinforcement Learning

Computer network defence is a complicated task that has necessitated a high degree of human involvement. However, with recent advancements in machine learning, fully autonomous network defence is becoming increasingly plausible. This paper introduces an end-to-end methodology for studying attack strategies, designing defence agents and explaining their operation. First, using state diagrams, we visualise adversarial behaviour to gain insight about potential points of intervention and inform the design of our defensive models. We opt to use a set of deep reinforcement learning agents trained on different parts of the task and organised in a shallow hierarchy. Our evaluation shows that the resulting design achieves a substantial performance improvement compared to prior work. Finally, to better investigate the decision-making process of our agents, we complete our analysis with a feature ablation and importance study.

==> evaluation.tex <==


%This section will discuss the evaluation metrics used, the performance of each subagent against their specific adversaries, and the overall model performance. 
In this section we evaluate the performance of our specialist subagents against the two adversaries. We further investigate the performance of the controller models. Finally, we evaluate the full defensive model capable of defending against either adversary. 
%
We use the model described in prior work~\cite{foley_autonomous_2022} as a baseline performance measure (baseline for brevity), as this has been established as state-of-the-art and achieved the best score in CAGE I. Because the scoring function assigns only penalty points (i.e., 0 is the theoretically maximum score), all the reported rewards are negative.
%The state-of-the-art winning PPO hierarchical with curiosity model from CAGE Challenge 1 was considered as the baseline. It has shown that our current model outperforms the baseline model to defend against attackers in CybORG simulation. 

%\begin{figure}
%    \centering
%    \includegraphics[width=1.0\textwidth]{images/subagents.pdf}
%    \caption{Mean, maximum and minimum reward of blue subagents against the %\code{BLineAgent} (left) and the \code{RedMeanerAgent} (right) over 10 million timesteps.}
%    \label{fig:sub_agent_training}
%\end{figure}

\begin{figure}[!t]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/mean_bline.eps}
  \caption{}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/mean_meander.eps}
  \caption{}
  \label{fig:sub2}
\end{subfigure}

\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/max_bline.eps}
  \caption{}
  \label{fig:sub3}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/max_meander.eps}
  \caption{}
  \label{fig:sub4}
\end{subfigure}

\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/min_bline.eps}
  \caption{}
  \label{fig:sub5}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/min_meander.eps}
  \caption{}
  \label{fig:sub6}
\end{subfigure}

\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/mean_sd_bline.eps}
  \caption{}
  \label{fig:sub7}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/mean_sd__meander.eps}
  \caption{}
  \label{fig:sub8}
\end{subfigure}
\caption{Mean, maximum and minimum reward of blue subagents against the \code{BLineAgent} (left) and the \code{RedMeanerAgent} (right) over 10 million timesteps.}
\label{fig:sub_agent_training}
\end{figure}



\subsection{Specialised Sub Agents}\label{ssec:eval_sub}
%\mf{this para is half included above, and the rest i am confused by}
%The model (blue agent) is trained to defend against the attackers (red agents) for 100 steps in each episode. Blue agent has penalty of -0.1 when the red agent has access to user hosts and operational hosts, and the penalty is -1 when it accesses operational and enterprise servers. Besides, some powerful actions like Impact and Restore cost -10 and -1 respectively. Maximising the reward function drives blue agents to keep attackers at hosts and protect servers by taking actions with less impact on the system. 

%The main performance metrics is the mean reward of an iteration of 40 episodes, which can reduce stochasticity in the model policy and the simulation environment in the result presentation. 
%The maximum and minimum reward of each training iteration were also recorded to understand the performance stability. The model with the highest mean reward was saved during training and then evaluated with 1000 episodes to collect more statistically representative mean and standard deviation of episode rewards.

\subsubsection{Training Results}
Figure~\ref{fig:sub_agent_training} shows the average reward of each defensive subagent as trained against the \code{BLineAgent} (left column), and the \code{MeanderAgent} (right column).
% 
The methods of AK and SR achieve peak rewards against the \code{BLineAgent} of -12.227 and -11.465 respectively, both of which are an improvement over the baseline~\cite{foley_autonomous_2022} PPO with curiosity based model, which achieves -13.475. Furthermore, removing curiosity negatively impacts the reward against the \code{BLineAgent}, as shown clearly in the max reward plot of Figure~\ref{fig:sub_agent_training}(c) 

%Meander or B-Line red agents more effective than the baseline. To defend against B-Line red agent, models using action knowledge (AK) and state representation (SR) method outperformed the baseline (-13.475) when comparing the best mean reward over all the training iterations, peaked at -12.227 and -11.465 respectively, where as Proximal Policy Optimisation (PPO) didn't have much improvement with best mean reward of -13.985. 
The difference in mean reward is explained by the maximum and minimum rewards. All models apart from PPO experience a first plateau in maximum reward of -9 and then step up to a second plateau of around -1. The SR agent finds the optimal policy earlier than the AK agent during training. In addition, the minimum rewards of the baseline and PPO model have greater variance than the SR and AK agents, and the AK agent has a marginally higher probability to score very poorly (i.e., below -300). Earlier optimal policy convergence and smaller policy variability makes the SR agent the best model against \code{BLineAgent} agent. This corroborates the standard deviation graph, and 1,000-episode evaluation results; in Table~\ref{table:sunagent_perf}, where the SR agent displays less negative reward and with a standard deviation that is only a fifth of the AK agent. 

Against the meander attacker the PPO and SR agents outperform the baseline (-24.384) with best mean rewards of -17.065 and -19.959 during training. Figure~\ref{fig:sub_agent_training} shows the advantage of using a PPO 3-layer architecture which results in higher min and max rewards with reduced variance.

\subsubsection{Specialist Agents}\label{ssec:specialists}
Here we evaluate the performance of our defensive subagents against their separate adversaries. We select the best performing agents from training for evaluation evaluate: PPO defence for the \code{RedMeander} and both the AK and SR defence for the \code{BLineAgent}. We evaluate each for 1,000 episodes of 100 steps and summarise our results in Table~\ref{table:sunagent_perf}. For completeness, we also cross-evaluate our agents against the adversary not seen during training.

Against the \code{RedMeander} adversary, PPO defence outperforms the baseline against both adversaries resulting in a mean score of -21.3 (improvement by a factor of 3.6) and a reduction in standard deviation by a factor of more than 9. This highlights the advantage of the increased depth of the neural network over the baseline. 

Against the \code{BLineAgent} adversary, we see that the SR agent is able to achieve a 1.5 times greater reward, with 4.89 times lower standard deviation. However, this comes at the cost of generality. A trend in all of the subagents is that when defending against previously unseen adversaries, the performance is significantly diminished. %For example, the SR agent achieves a reward 1.75 times worse than AK, 1.27 times worse than the baseline. 

%Against \code{BLineAgent}, the SR defence outperforms AK with 1.48 less penalty points and a standard deviation 4.89 times lower. Yet, while SR is a better defensive agent against the \code{BLineAgent} this comes at a cost of less generality, a trend we see in \emph{all} of the subagents. This is a significant difference in the reward as it results in worse mean reward for SR that is 1.75 times greater than AK, and 1.27 times greater than the baseline. 

%Our results support the need for an architecture beyond a single agent policy as defensive strategies differ significantly between the two adversaries. Note however, that the \code{MeanderAgent} defensive agents learn a more general policy than their \code{BLineAgent} counterparts. 


\begin{table}[]
\centering
{\footnotesize
\begin{tabular}{@{}llccccll@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Training\\ Adversary\end{tabular}}              & \multirow{2}{*}{Defensive Model} & \multicolumn{2}{c}{\texttt{BLineAgent}}                                                                                                                       & \multicolumn{2}{c}{\texttt{MeanderAgent}}                                                                                                                     & \multicolumn{2}{c}{Mean}                                                                                              \\ \cmidrule(l){3-8} 
 &                                  & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Mean \\ Reward\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Standard\\ Deviation\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Mean \\ Reward\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Standard \\ Deviation\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Mean \\ Reward\end{tabular} & \begin{tabular}[c]{@{}l@{}}Standard\\  Deviation\end{tabular} \\ \midrule
\texttt{MeanderAgent}  & PPO    &  \textbf{-24.91}  & \textbf{9.21}  &   \textbf{-17.71}   &   \textbf{5.06}       &  \textbf{-21.31}   &  \textbf{7.43}  \\ 
                & baseline     & -123.91    & 229.59     &  -30.39    & 47.74   &   -77.15  &      165.82    \\ \hline
\multirow{3}{*}{\texttt{BLineAgent}} & AK    & -14.43   & 30.28     &  \textbf{ -145.26}   &  \textbf{123.92}     &    \textbf{-79.84}  &    \textbf{90.20}     \\ 
                                          & SR     & \textbf{-12.95}    & \textbf{6.19}     &  -269.64   &    235.24    &   -139.29    &   166.40  \\ 
                                          & baseline    & -16.80  & 21.12    &   -201.13   &  143.40  &   -108.96   &      102.49       \\ \bottomrule
                                          
\end{tabular}}
\vspace{+2mm}
\caption{The performance of the defensive subagents against their corresponding adversaries. Evaluated on 1,000 episodes of 100 timesteps each.}\label{table:sunagent_perf}

\end{table}


\subsection{Controller Models}\label{ssec:eval_control}
As seen in Section~\ref{ssec:specialists}, the defensive subagents do not generalise well beyond the adversaries that they are trained against.

%are able to handle the
%adversaries that they are trained against but . %Thus our architecture utilises a hierarchical controller that selects one of the trained subagents. 
%While~\cite{foley_autonomous_2022} introduced a deep learning based approach we argue that this is unable to truly capture the subtly in the adversaries. Thus to remove this problem we have used explainablity methods to model the adversaries and introduce two new controller architectures: Heuristic and Bandit. 
To address this, Sections~\ref{ssec:heuristic_controller} and~\ref{ssec:bandit_controller}
introduce two new controller architectures: Heuristic and Bandit. Here we evaluate the ability to correctly predict the adversary within the first four timesteps of an episode (as our controllers predict the adversary on the fourth timestep). For each episode, we randomly sampled one of the two red adversaries (i.e., 50\% probability of selecting \code{BLineAgent}).

%As the baseline model (PPO with curiosity) predicts the adversary at every timestep we also include the prediction accuracy over 100 steps, taking the mode of the predictions.

%It is found that Heuristic and Bandit controllers have improved the overall model performance when Meander and B-Line red agents appear randomly. 
Table~\ref{table:controller_pred} shows that the baseline model has strong biases on selecting the \code{BLineAgent} agent. To investigate further, we let the baseline agent make predictions on each timestep until the end of the episode (c.f. only guessing after the 4th timestep). As seen in Table~\ref{table:controller_pred}, the repeated guesses significantly reduced bias but accuracy remained low.

In contrast, neither our bandit or heuristic controller exhibit this bias and can perfectly predict the correct attacker type. 

%After combining them with our specialist agents and evaluating for 1,000 episodes, the Heuristic and Bandit controller demonstrated an almost identical performance when defending both against \code{RedMeander} and \code{BLineAgent} agents: $-13.0 \pm 6.28$ against B-Line and $-17.56 \pm 4.51$ against Meander.

\begin{table}[]
\centering
\begin{tabular}{@{}l|cc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Controller Agent}} & \multicolumn{2}{c}{Prediction Accuracy} \\ \cmidrule(l){2-3} 
\multicolumn{1}{c|}{}                                  & \texttt{BLineAgent}   & \texttt{RedMeander}   \\ \midrule
PPO with curiosity (4 steps)                           & 76.8\%              & 0.0\%               \\
PPO with curiosity (100 steps)                         & 30.3\%              & 42.9\%              \\
Heuristic                                              & 100.0\%             & 100.0\%             \\
Bandit                                                 & 100.0\%             & 100.0\%             \\ \bottomrule
\end{tabular}
\vspace{+2mm}
\caption{Controller performance taken over 1,000 episodes of 4 steps, except in the case of PPO with curiosity (100 steps) which predicts the adversary at each timestep.}\label{table:controller_pred}
\end{table}

%Sections~\ref{ssec:eval_sub} and~\ref{ssec:eval_control} describe how well the individual elements of the hierarchical model compare,

\subsection{Hierarchical Defensive Model}\label{ssec:eval_complete}
 Here we evaluate the complete defensive model. Table~\ref{table:overall_eval} reports the mean and standard deviation for the `best pair' combinations of subagents as determined by our evaluation in Section~\ref{ssec:eval_sub} ( i.e., PPO for \code{MeanderAgent}, and AK or SR for \code{BLineAgent}).

We observe that the subagents play a significant role in the improvement over the baseline. Over episodes of 100 timesteps, we are able to improve the result by at least 30\% for the \code{BLineAgent} and 170\% for \code{MeanderAgent}. 

%This is unsurprising as they both achieve perfect prediction accuracy. Note that there is an improvement from using these controllers, they
The lowest reward values are split evenly between the Heuristic and Bandit controllers. These models outperform the PPO controller models regardless
of the subagents in four of the six combinations of adversary and episode length. 

%Figure~\ref{fig:sub_agent_training} shows the differentiated performance when defending against \code{MeanderAgent}. 
\code{MeanderAgent} performance is improved by 11.7\%, which is more significant than \code{BLineAgent} (only improved by 1\%) when using Bandit or Heuristic controller. Table~\ref{table:sunagent_perf} indicates that models trained with \code{BLineAgent} perform poorly on \code{MeanderAgent}. This can be explained by the fact that \code{BLineAgent} has more information about the network, so its behaviour is more predictable. In contrast, \code{MeanderAgent}'s actions have more randomness.

% \mf{insert look at how good it is tho}

%We then evaluate the complete defensive model to determine its overall performance. 
%  controller evaluation table
\begin{table}[]
\centering{\fontsize{6.7pt}{8pt}\selectfont
\begin{tabular}{@{}p{1.8cm}p{1.7cm}cccccc@{}}
\toprule
\multirow{2}{*}{Controller}              & \multirow{2}{*}{Subagents} & \multicolumn{2}{c}{\texttt{30  steps}}                                                                                                                       & \multicolumn{2}{c}{\texttt{50 steps}}                                                                                                                     & \multicolumn{2}{c}{100 steps}                                                                                              \\ \cmidrule(l){3-8} 
 &                                  & \texttt{\fontsize{6.7pt}{8pt}\selectfont BLineAgent} & \multicolumn{1}{c}{\texttt{\fontsize{6.7pt}{8pt}\selectfont MeanderAgent}} & \multicolumn{1}{c}{\texttt{\fontsize{6.7pt}{8pt}\selectfont BLineAgent}} & \multicolumn{1}{c}{\texttt{\fontsize{6.7pt}{8pt}\selectfont MeanderAgent}} & \texttt{\fontsize{6.7pt}{8pt}\selectfont BLineAgent} & \texttt{\fontsize{6.7pt}{8pt}\selectfont MeanderAgent} \\ \midrule
\multirow{2}{*}{Bandit}  & PPO + AK    & \textbf{-3.56$\pm$2.03} &  \textbf{-6.80$\pm$1.40}   &   -6.79$\pm$13.00      &  -10.10$\pm$2.30   &   -13.54$\pm$15.95 & \textbf{-17.30$\pm$4.27}\\ 
                & PPO + SR     &  -3.62$\pm$2.04    & -6.88$\pm$1.42     &   -6.26$\pm$3.18   & -10.06$\pm$2.15   &  \textbf{-13.00$\pm$6.28}   &    -17.56$\pm$4.51      \\ \midrule
\multirow{2}{*}{Heuristic}  & PPO + AK   &  -3.56$\pm$2.04  & \textbf{-6.80$\pm$1.40 }&    -6.79$\pm$13.00   &  \textbf{ -9.96$\pm$2.33 }  &  -14.07$\pm$27.73   &  -17.57$\pm$4.82  \\ 
                & PPO + SR     & -3.71$\pm$2.09    & -6.86$\pm$1.48    & \textbf{ -6.17$\pm$3.40}    & -10.04$\pm$2.32   &  -13.06$\pm$6.14   &    -17.32$\pm$4.35      \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} Baseline  \\ (PPO Controller)\end{tabular}} & PPO + AK  &  -4.35$\pm$2.42 & -7.19$\pm$1.69   &  -7.45$\pm$4.27   &   -10.84$\pm$2.62    &  -14.97$\pm$8.09   &    -19.33$\pm$5.38     \\ 
                    & PPO + SR    & -3.95$\pm$2.18  &  -7.36$\pm$1.74   &  -6.38$\pm$3.20   &  -11.33$\pm$3.00  &   -13.14$\pm$6.45  & -21.21$\pm$6.10            \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} Baseline  \\ (PPO Controller)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} Baseline  \\ (PPO subagents)\end{tabular}} &   4.82$\pm$4.22 & -8.78$\pm$3.21   & -9.20$\pm$16.01     &   -19.00$\pm$20.86    &    -18.49$\pm$34.40 &  -47.60$\pm$88.16       \\ 
\\
                                            
                    \bottomrule
                                          
\end{tabular}}
\vspace{+2mm}
\caption{Performance of all subagents-controller combinations, evaluated over 1,000 episodes with a length of 30, 50 and 100 steps each.}\label{table:overall_eval}

\end{table}



% \texttt{\begin{tabular}[c]{@{}l@{}}PPO \\ (baseline)\end{tabular}} 
